Long Working Distance Apodized Grating Coupler

We design a focusing grating coupler by a simultaneous apodization of the filling factor and the period. In addition to in plane focusing to the input waveguide providing a total length of less than 70{\mu}m, a further apodization of the curvature allows out of plane focusing into a fiber set 150{\mu}m away from the grating surface. The design is proposed for novel semiconductor on insulator waveguides such as GaInP. The coupling efficiency is calculated from two dimensional simulation which is about 45%.

==> appendice.tex <==
\section*{Fiber Numerical Aperture (NA) in Radians}
	\label{sec:numerical_aperture}
	
	Numerical aperture of a standard single mode fiber (SMF) measured at $1 \%$ power level of an 1D far-field scan at 1550 nm is $0.14$. At $1 \%$ power level of the Gaussian output beam $ exp ( - 2 (\frac{w_{1 \%}}{\sigma})^2 ) = 0.01$ where $w_{1 \%}$ is the half beam width. At the half of the maximum power level $  exp ( - 2 (\frac{w_{FWHM}/2}{\sigma}) ^2 ) = 1/2 $ where $w_{FWHM}$ is the full width at the half of maximum power. We can readily obtain that $w_{1 \%} = \sigma$ and $w_{FWHM} = \sigma \sqrt{2ln(2)}$. Width at one percent power level is related to the  $w_{FWHM}$ by the factor $\frac{w_{FWHM}}{w_{1 \%}} = sqrt{\frac{2ln(2)}{ln(10)}} = 0.775925$.  To match the fiber mode, the output beam from the grating should achieve the full width  $w_{FWHM} \sim 0.1$ radians. 

==> sim_method.tex <==
\label{subsec:CAMFR}
It is well known that the profile of the radiation emerging from an uniform grating is a decaying exponential \textcolor{red}{which overlaps poorly with the close to Gaussian profile of the fiber mode, leading to a limited coupling efficiency \cite{waldhausl1997efficient,bates1993gaussian}.} This issue is solved in an apodized grating, where the parameters are modulated spatially in order to tailor the emerging radiation to the fiber mode. Another improvement consist in adjusting the transverse profile by tapering the width of the mode from the size of a narrow rib waveguide to that of the fiber\cite{van2007compact}, as shown in fig. \ref{fig:mode_match}(b). More precisely, the grating consists in arc shaped ribs with radius $R(x)$. A suitable choice of the parameters, which will be discussed here below, ensures that a Gaussian beam emerges from the structure and that its profile matches the fiber mode. If the fiber is not in contact with the grating, an additional curvature of the phasefront in introduced, as shown in fig. \ref{fig:mode_match}

	%\begin{figure}[ht!]
	%	\centering\includegraphics[width=2.5in]{khan2}
	%	\caption{In-plane focusing taper for mode matching in the transverse direction.}
		%\label{fig:problem_exp}
	%\end{figure}
We start with

%For modeling of the devices, eigen mode expansion method and 3D finite difference time domain (FDTD) method were used. For the 2D modeling of the grating couplers the software package Cavity Modeling Framework was used, popularly known as CAMFR, developed by P. Bienstman from Ghent University \cite{bienstman2008camfr}. An example code from \cite{taillaert2004grating} was adapted and modified for the modeling of our grating designs. Figure \ref{fig:bragg_cond}(a), shows the basic structure for 2D CAMFR simulation where the blue lines indicate simulation boundary. 3D FDTD method was used to model the behavior of designed grating couplers using in-house FDTD simulation tool which has been rigorously studied and results produced by it have been verified to be accurate \cite{NVQTran2011}. 
